Inferring unknown biological function by integration of GO annotations and gene expression data

Characterizing genes with semantic information is an important process regarding the description of gene products. In spite that complete genomes of many organisms have been already sequenced, the biological functions of all of their genes are still unknown. Since experimentally studying the functions of those genes, one by one, would be unfeasible, new computational methods for gene functions inference are needed. We present here a novel computational approach for inferring biological function for a set of genes with previously unknown function, given a set of genes with well-known information. This approach is based on the premise that genes with similar behaviour should be grouped together. This is known as the guilt-by-association principle. Thus, it is possible to take advantage of clustering techniques to obtain groups of unknown genes that are co-clustered with genes that have well-known semantic information (GO annotations). Meaningful knowledge to infer unknown semantic information can therefore be provided by these well-known genes. We provide a method to explore the potential function of new genes according to those currently annotated. The results obtained indicate that the proposed approach could be a useful and effective tool when used by biologists to guide the inference of biological functions for recently discovered genes. Our work sets an important landmark in the field of identifying unknown gene functions through clustering, using an external source of biological input. A simple web interface to this proposal can be found at http://fich.unl.edu.ar/sinc/webdemo/gamma-am/.

==> sup_material.tex <==
\section*{Supplementary Material}
\subsection*{Full results for YEA dataset}
%\input{table_supp_material_yea}
\input{table_supp_material_yea2}
\newpage

\subsection*{Full results for ARA dataset}
\input{table_supp_material_ara}


==> sup_material_2.tex <==
\subsection*{ARA results}
For ARA dataset, an analogous procedure to the YEAST dataset was performed. Expression distance and semantic distance matrices were built and both the \disc{} and the $\gamma$-tuning method were applied. Histograms for expression distance and semantic distance matrices are shown in Figure \ref{fig:02-ara} before applying the \disc{} method and in Figure \ref{fig:03-ara} after the application of this method. Application of the $\gamma$-tuning method is shown in Figure \ref{fig:results-gamma-measure-ara}.

\begin{figure}[t!]%figure2
\centerline{\includegraphics[scale=0.23]{graficos/histogramas_01_ara.pdf}}
\caption{Original distance histograms distributions for the ARA gene dataset. Expression-based pairwise distances (left) and semantic-based pairwise distances (right).}\label{fig:02-ara}
\end{figure}

\begin{figure}[t!]%figure2
\centerline{\includegraphics[scale=0.23]{graficos/histogramas_02_ara.pdf}}
\caption{Histograms for the ARA pairwise distances from Figure \ref{fig:02-ara} after applying the \disc{} method. Expression-based pairwise distances (left) and semantic-based pairwise distances (right).}\label{fig:03-ara}
\end{figure}

\begin{figure*}[t!]%figure1
\centerline{\includegraphics[scale=0.48,trim=0 20 0 50, clip]{resultados/salida_dist_schlicker_v7_ara.pdf}}
\caption{Results for the $\gamma$-tuning method on the ARA dataset.} \label{fig:results-gamma-measure-ara}
\end{figure*}



Measures for validation were also calculated on this dataset. Results for $BHI$ and $BC$ on the partition $G^{A_2 \rightarrow A_1}$ are shown in Table \ref{tab:results-bhi-gamma-tuning-ara}. The first column indicates the method applied. For the $\gamma$-tuning method, which is shown in the first row, an appropriate $\gamma$ value of 0.75 was used for a proportion of $A1/A2 = 50/50$, as resulting from Figure \ref{fig:results-gamma-measure-ara}. Results obtained when applying the \disc{} method are shown in the second row (Yes), and when not applying this method are shown in the third row (No). In both cases a gamma value of $\gamma = 0.50$ was used.

It can be seen from the table that, for both measures, the $\gamma$-tuning method clearly provides the best results. This shows that higher biological quality is reached on the partition $G^{A_2 \rightarrow A_1}$ with this method when it is compared to the \disc{} method, analogously to the performance measures obtained on the YEAST dataset.

In order to evaluate the clustering quality of Step 2, recall was also calculated for this dataset. An annotation count has also been calculated in this case, as shown in Table \ref{tab:count-etiquetas-ara}. The first and second columns describe the GO label, and the third column shows the number of genes in the dataset annotated with the corresponding GO label. As it can be seen in the table, there is not a noticeable difference among the label counts, and therefore a more homogeneus label distribution is found in this case, with no distinguishable popular labels to consider. It should be noted here that this is probably due to the fact that Arabidopsis is a model specie and it is thoroughly studied in literature, and therefore its GO terms are well annotated. Thus, the recall calculation should not be very much affected by the removal of popular terms. Anyway, the first three most used labels (regulation of transcription, DNA-templated, response to salt stress and oxidation-reduction process) were removed to make a comparison against the full label set. Results are shown in Table \ref{tab:accuracy_ara}. The first row shows recall for the classic approach, while the second row shows recall considering complete semantic information, and the third row shows the recall with our approach. In the second column, it can be seen that the value of 0.052 obtained with \gss{} is very close to the best possible value of 0.071, and fairly better than the value of 0.033 obtained by the classic approach. Columns comparing these values by calculating differences with respect to the complete information case are also provided in the third column. Here, while our method has a percentual error of 26.76\% with respect to the best case, the classical approach has the double of percentual errors in assigning labels to unknown genes. Recall without taking into account the first labels (fourth column and fifth columns) show similar results, proving the effectiveness of our method when applied to this dataset as well. 

\input{table_bhi_ara_gamma_tuning}

\input{table_count_etiquetas_ara}

\input{table_accuracy_ara_sup}

\dif{Clustering performance was also evaluated for this dataset, comparing the clustering in Step 2 to the SOM-based co-clustering in terms of $BHI$ and $BC$. Results are shown in Table \ref{tab:results-comparison-ara}. It can be seen that the clustering quality of \gss{} outperforms the SOM co-clustering for this dataset as well. Our method yields the best $BHI$ (0.12) compared to the lower values (0.06 and 0.10) for the SOM-based method. Similar results are reached in terms of $BC$, with the best value (0.59) against the less compact results for the SOM approach.}

\input{table_comparacion_som_ara_sup}

%Regarding biological quality, Table \ref{tab:results-test-ara} shows the results of our method in the third row. The first row shows the results for the best possible case, using complete semantic information, whereas the second row shows the values for the classical approach. It can be seen that, for both measures, the application of the $\gamma$-tuning method with an appropriate $\gamma$ value used to balance the amount of the expression and semantic GO-based data is significantly close in terms of biological quality to the best possible values of both performance measures. For $BHI$, the value of 0.14 obtained with our method is remarkably near to the best value of 0.15, representing a major improvement to the value of 0.05 obtained when applying the classical method. Similar results are obtained for BC, where a value of 0.60 for our method is very close to the best value of 0.59 obtained with full semantic information and indicates a considerable higher compactness than the value of 0.82, which was obtained with $A \cup B$ with $\gamma = 0$. 
%The quality of Step 2 was also evaluated with the FM index. A random assignment and our approach were compared against the best possible case, obtaining the values 0.12 and 0.15, respectively. These results show a similarity improvement of nearly 25\%  between the partition obtained with \gss{} and the partition that would be obtained with complete semantic information.

%\input{table_test_ara}

%The appropriate $\gamma$ value of 0.75 obtained by the $\gamma$-tuning method is used as an input to Step 2 of \gss{}. The resulting partition $G^{B \rightarrow A}$ is then evaluated in terms of biological quality upon $BHI$ and $BC$. Table \ref{tab:results-test-ara} shows the results of our method in the third row. The first row shows the results for the best possible case, using complete semantic information, whereas the second row show the values for the classical approach.

%It can be seen that, for both measures, the application of the $\gamma$-tuning method with an appropriate $\gamma$ value used to balance the amount of the expression and semantic GO-based data is significantly close in terms of biological quality to the best possible values of both performance measures. For $BHI$, the value of 0.14 obtained with our method is remarkably near to the best value of 0.15, representing a major improvement to the value of 0.05 obtained when applying the classical approach. Similar results are obtained for BC, where a value of 0.60 for our method is very close to the best value of 0.59 obtained with full semantic information and indicates a considerable higher compactness than the value of 0.82, which was obtained with $A \cup B$ with $\gamma = 0$.

%The quality of Step 2 was also evaluated with the FM index. A random assignment and our approach were compared against the best possible case, obtaining the values 0.12 and 0.15, respectively. These results show a similarity improvement of nearly 25\%  between the partition obtained with \gss{} and the partition that would be obtained with complete semantic information.

%\input{table_input_assignment_ara}



A detailed example regarding the automatic annotation of genes is also presented for this dataset. 
%Table \ref{tab:input-enrichment-analysis-ara} shows input genes from $A$ and $B$ dataset. 
Table \ref{tab:enrichment-analysis-ara} shows the output for the enrichment analysis procedure. Results for cluster \clusterara{} are shown in table \ref{tab:validation-assignment-procedure-ara}, with matching terms shown in bold. Results are very promising for this example. Several actual GO terms for a subset of assigned genes matched exactly cluster terms obtained through enrichment analysis. This is shown graphically in Figure \ref{fig:mapa_go_ara}. Relative location of inferred terms in GO is shown in the figure, analogously to the example for the YEAST dataset. Matching terms are very close to the rest of the assigned terms. Original terms from $B$ are also close (as siblings) to assigned terms. From these results, it can be seen that there are many terms from $B$ that are correctly inferred by our approach. Furthermore, also for this dataset, it can be clearly seen that, for original terms from $B$ there is a remarkable closeness between them and the terms assigned by the procedure.


%

%
\input{table_enrichment_analysis_ara}



\input{table_validations_assignment_procedure_ara}



%









\begin{sidewaysfigure*}
%\begin{figure*}[t!]%figure1
\centerline{\includegraphics[width=\textwidth]{resultados/GO_example_cluster_arabidopsis.pdf}}
\caption{Inferred terms in the Gene Ontology for gene \geneexampleara{} from cluster \clusterara{} of the ARA dataset: assigned terms (dashed line), matching terms (ellipse), original B terms (thick line).} \label{fig:mapa_go_ara}
%\end{figure*}
\end{sidewaysfigure*}

